SEAM: A Self-Evolving and Adaptive Probing Framework for Automatic MLLM Hallucination Evaluation

The severe susceptibility of multimodal large language models (MLLMs) to hallucinations poses a critical threat to their reliability, making a rigorous evaluation framework indispensable. However, existing evaluation pipelines largely rely on predefined test items, suffering from high construction costs, rapid obsolescence as MLLMs evolve, and ineffectiveness in probing model-specific weaknesses. To address these limitations, we propose SEAM, a self-evolving and adaptive probing framework for automatic MLLM hallucination evaluation. Specifically, SEAM introduces a composable Hallucination Probe Construction Library comprising ten hallucination-probing skills, three elicitation wrappers, and five question formats. Building on this library, SEAM establishes a dual-loop framework. In the inner loop (adaptive probing), skill-guided visual analysis, question composition, and hierarchical quality verification are coordinated with verifier and target-response feedback to refine test items and uncover model-specific hallucinations. In the outer loop (skill evolution), a skill updater distills historical probing trajectories into localized, reusable rule updates, which undergo held-out validation and are frozen before testing. Driven by these innovative structural designs, SEAM establishes an automated and self-evolving evaluation paradigm. Experiments across four target MLLMs and ten hallucination types demonstrate that SEAM substantially outperforms representative static benchmarks, achieving an 89.2\% relative improvement in mean valid hallucination discovery rate across 12 matched comparisons.

==> sec/3_finalcopy.tex <==
\section{Method}
\label{sec:method}
\subsection{Overview}
\label{sec:overview}

\begin{figure*}[!t]
    \centering
    \includegraphics[
        width=\textwidth
    ]{Figures/model.pdf}
    \caption{
    Overview of SEAM.
    }
    \label{fig:overview}
\end{figure*}

We present \textbf{SEAM}, a dynamic multimodal hallucination evaluation framework combining adaptive probing with skill evolution. As illustrated in Figure 1, given an image pool and a target MLLM, SEAM comprises three components. The \textbf{Shared Skill Library} provides probing skills covering ten hallucination types, together with elicitation wrappers and question formats. \textbf{Adaptive Hallucination Probing} generates and verifies questions under skill guidance, then refines them using quality and target-response feedback within a predefined attempt budget. \textbf{Evidence-Guided Skill Evolution} distills experience from training trajectories and proposes local skill edits, accepting updates or retaining the original skills based on independent validation. The library is frozen before testing. Finally, SEAM produces valid hallucination cases and reports the question quality pass rate and valid hallucination discovery rate (VHDR), forming a closed loop for uncovering target-model weaknesses and improving probing strategies under quality and budget constraints.


\definecolor{cvprgray}{HTML}{F2F4F7}

\subsection{Shared Skill Library}
\label{sec:skill_library}
% Required packages: \usepackage{booktabs,tabularx,array}
\begin{table}[!htbp]
\centering
\caption{Hallucination types covered by the probing skills in SEAM. }
\label{tab:hallucination_skills}
\begingroup
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabularx}{\linewidth}{
    @{}
    l
    l
    >{\raggedright\arraybackslash}X
    @{}
}
\toprule
\textbf{ID} & \textbf{Probing Skill} & \textbf{Target Hallucination Mechanism} \\
\midrule
\rowcolor{cvprgray}
\multicolumn{3}{@{}l}{\textbf{V. Visual Evidence}} \\
V1 & Object Insertion & Claims objects absent from the image. \\
V2 & Attribute Shift & Alters color, shape, material, size, or pose. \\
V3 & Perceptual Relation & Distorts visible spatial or contact relations. \\
V4 & Counting Error & Misreports counts of visible objects. \\
V5 & Text/OCR Manip. & Misreports visible text, digits, or signs. \\
\addlinespace[1.5pt]
\rowcolor{cvprgray}
\multicolumn{3}{@{}l}{\textbf{C. Contextual Knowledge}} \\
C1 & Cognitive Relation & Misreads causal, social, or action relations. \\
C2 & Factual Conflict & Links visible entities to false external facts. \\
C3 & Commonsense & Violates physical, biological, or social norms. \\
\addlinespace[1.5pt]
\rowcolor{cvprgray}
\multicolumn{3}{@{}l}{\textbf{E. Evidence Boundary}} \\
E1 & Reasoning Overreach & Infers unobservable intent, cause, or future. \\
E2 & Unverifiable Infer. & Answers definitely under blur or occlusion. \\
\bottomrule
\end{tabularx}
\endgroup
\end{table}
SEAM maintains a shared skill library comprising hallucination probing skills $\mathcal{S}$, elicitation wrappers $\mathcal{W}$, and question formats $\mathcal{F}$. These resources jointly guide visual analysis, question composition, verification, and refinement.

\paragraph{Hallucination probing skills.}
As summarized in Table~\ref{tab:hallucination_skills}, $\mathcal{S}$ contains 10 skills grouped into Visual Evidence, Contextual Knowledge, and Evidence Boundary. Each skill combines a fixed hallucination-type definition with editable probing rules that guide visual analysis, question construction, and reference-answer verification. Each question targets a single hallucination skill $s_i\in\mathcal{S}$. The outer loop updates the probing rules while preserving the type definitions.

\paragraph{Elicitation and presentation.}
The wrapper library $\mathcal{W}$ specifies three elicitation strategies: prior induction, which encourages an unsupported interpretation; false presupposition, which presents an incorrect claim as established; and fabricated authority, which attributes an unsupported claim to an apparently credible source. The question-format library $\mathcal{F}$ includes multiple-selection, single-choice, fill-in-the-blank, true/false, and open-ended formats, each with a verifiable reference answer or evaluation criterion.

\paragraph{Configuration constraints.}
Each skill is assigned a wrapper through a fixed mapping $b:\mathcal{S}\rightarrow\mathcal{W}$. We define $\Omega\subseteq\mathcal{S}\times\mathcal{W}\times\mathcal{F}$ as the set of compatible configurations satisfying $w=b(s)$. For task $i$, the probing configuration is
\begin{equation}
z_i=(s_i,w_i,f_i)\in\Omega,
\qquad w_i=b(s_i),
\end{equation}
where $f_i\in\mathcal{F}$ is compatible with the selected skill and its assigned wrapper. The configuration remains fixed across attempts within each task. Wrapper definitions and bindings, format specifications, and compatibility constraints remain unchanged during skill evolution.

\subsection{Adaptive Hallucination Probing Pipeline}
\label{Adaptive Hallucination Probing Pipeline}

The inner loop constructs and refines questions to uncover target-specific
hallucinations under a fixed attempt budget.
As shown in Figure~1, it combines skill-guided visual analysis,
question composition, hierarchical verification, target-model evaluation,
and feedback-guided refinement.

For each image $x_i$, the Visual Analysis Agent retrieves an applicable
skill from the Shared Skill Library and performs skill-specific visual
analysis. The Question Composer then generates a candidate question
and its reference answer. The Hierarchical Question Verifier checks
the candidate before it is submitted to the target MLLM $\mathcal{M}$,
whose response is assessed by the Hallucination Judge.
If the question fails quality verification or the response does not
exhibit a hallucination, the Failure-Aware Refinement Agent uses the
corresponding feedback to revise the question, provided that budget
remains. Probing stops when a quality-approved question elicits a
hallucination or the attempt budget $K$ is exhausted.
We use $K=2$, allowing an initial attempt and at most one
feedback-guided revision. The skill configuration remains fixed
throughout each task.

\paragraph{Visual Skill Analysis Agent.}
\label{sec:visual_skill_agent}

A hallucination skill is meaningful only when the image satisfies its visual
preconditions. For example, counting requires distinguishable instances,
attribute manipulation requires observable properties, and OCR evaluation
requires legible text. The \emph{Visual Skill Analysis Agent} therefore
verifies a designated skill or selects an applicable one when no trusted
skill label is available:
\begin{equation}
(s_i,a_i)
=
\operatorname{VSA}
\left(
x_i,m_i,\tilde{s}_i;\mathcal{S}
\right),
\end{equation}
where $s_i\in\mathcal{S}$ is the verified or selected skill and $a_i$ is its
skill-specific visual analysis. An image--skill pair that fails the required
visual preconditions is excluded from subsequent construction.

For \emph{V5 Text/OCR Manipulation}, for example, $a_i$ identifies
text-bearing regions and transcribes only legible content. Metadata may guide
the analysis, while all evidential claims and reference answers are checked
by the \emph{Hierarchical Question Verifier}.

\paragraph{Hallucination-Eliciting Question Composer.}
\label{sec:question_composer}

Identifying an applicable skill does not by itself yield a diagnostic
question: the relevant visual evidence must be converted into a concrete
probe with an appropriate elicitation strategy and answer interface. The
\emph{Hallucination-Eliciting Question Composer} therefore instantiates the
selected skill into a complete and verifiable question under a compatible
wrapper and format.

Given $x_i$, $s_i$, and $a_i$, the Composer selects a compatible wrapper
$w_i\in\mathcal{W}$ and question format $f_i\in\mathcal{F}$, yielding the
configuration $z_i\in\Omega$. The configuration is held fixed across
construction attempts. At attempt
$t\in\mathcal{A}_i\subseteq\{1,2\}$, the Composer, implemented using a VLM,
generates
\begin{equation}
u_{i,t}
=
\operatorname{HEQC}
\left(
x_i,a_i,z_i,\eta_{i,t}
\right)
=
\left(
q_{i,t},
\rho_{i,t},
y_{i,t}^{\star}
\right),
\end{equation}
where $q_{i,t}$ is the candidate question, $\rho_{i,t}$ is the instantiated
elicitation content, and $y_{i,t}^{\star}$ is the evidence-grounded reference
answer. The revision input satisfies $\eta_{i,1}=\varnothing$; when a retry
is triggered, $\eta_{i,2}$ contains quality-diagnostic or target-oriented
feedback.

Generation follows three constraints: the question must isolate the failure
mechanism of $s_i$; the wrapper may increase elicitation pressure without
adding another hallucination mechanism; and the format must support a reliably
verifiable answer or evaluation criterion.

\paragraph{Hierarchical Question Verifier.}
\label{sec:hierarchical_question_verifier}

We assess generated questions through two-stage quality verification, independent of target-model responses and hallucination judgments. The verifier receives the original image, question, reference answer, and specifications of the assigned skill, wrapper, and answer format.

The first stage checks four validity conditions: skill alignment, wrapper compliance, format validity, and reference-answer correctness. The answer check decomposes the reference answer into key claims and verifies each against the image and task-permitted auxiliary evidence. We set $V_{i,t}=1$ when all four conditions hold and $V_{i,t}=0$ when any condition fails. Otherwise, unresolved evidence triggers a separate review status rather than a definitive validity label.

Only candidates with $V_{i,t}=1$ receive second-stage scores. The rubric evaluates two dimensions: plausibility, measuring the relevance of the probing target to the image and the naturalness of its presentation; and diagnosticity, measuring whether potential errors can be attributed to the assigned hallucination mechanism while minimizing ambiguity and confounding factors. Each dimension receives a score from 0 to 2:
\begin{equation}
R_{i,t}=\sum_{d\in\mathcal{D}}r_{i,t}^{d},
\qquad
\mathcal{D}=\{\mathrm{plaus},\mathrm{diag}\},
\quad
r_{i,t}^{d}\in\{0,1,2\}.
\end{equation}
For candidates with resolved validity decisions, the final quality decision is
\begin{equation}
Q_{i,t}=
\begin{cases}
\mathbf{1}[R_{i,t}\geq3]\,
\mathbf{1}[\min_{d\in\mathcal{D}}r_{i,t}^{d}\geq1],
& V_{i,t}=1,\\
0, & V_{i,t}=0.
\end{cases}
\end{equation}
Candidates awaiting review remain pending until the required evidence is resolved. The verifier also returns structured evidence, identified defects, and requests for additional evidence as feedback $\phi_{i,t}$, supporting question refinement and subsequent skill updates. Only candidates with $Q_{i,t}=1$ are evaluated on the target MLLM.


\paragraph{Target-Model Evaluation.}
\label{sec:target_model_evaluation}

Question validity alone does not indicate whether a candidate can expose an
actual weakness of the target VLM. SEAM therefore evaluates every
quality-approved question on the target model and uses an independent
\emph{Hallucination Judge} to quantify the resulting failure severity.
% [M-06] 统一公式 (7) 中的目标模型符号为花体 \mathcal{M}，并显式写出 \eta_{i,2} 的双路路由与有效性优先规则 (Q_{i,2}=1)
\todo[inline]{Unify target model symbol to }%\mathcal{M} in Eq. (7), explicitly connect \eta_{i,2} routing to \phi_{i,1} and F_{i,1}^{tar}, and state validity-first rule (Q_{i,2}=1).}

For each quality-approved candidate, the target VLM $\mathcal{M}$ produces
\begin{equation}
\hat{y}_{i,t}
=
\mathcal{M}
\left(
x_i,q_{i,t}
\right).
\end{equation}
The \emph{Hallucination Judge} assigns
\begin{equation}
j_{i,t}
=
J_{\mathrm{hall}}
\left(
x_i,
q_{i,t},
y_{i,t}^{\star},
\hat{y}_{i,t}
\right)
\in\{1,\ldots,10\},
\end{equation}
using the image, question, evidence-grounded reference answer, and
target-model response. Scores of 1--3 indicate clear hallucination, scores of
4--6 indicate ambiguous or partially grounded responses, and scores of 7--10
indicate correct answers or explicit rejection of an unsupported premise.
Lower scores indicate stronger hallucination elicitation.

For threshold $k$, the elicitation outcome is
\begin{equation}
H_{i,t}^{(k)}
=
\begin{cases}
\mathbf{1}
\left[
j_{i,t}\leq k
\right],
& Q_{i,t}=1,\\
0,
& Q_{i,t}=0.
\end{cases}
\end{equation}
The indicators $H_{i,t}^{(1)}$ and $H_{i,t}^{(3)}$ correspond to HER@1 and
HER@3, respectively. Under the primary criterion, hallucination is
successfully elicited when $H_{i,t}^{(3)}=1$.

% %[G-03] 在第 3.3 节 Target-Model Evaluation 结尾说明 H_{i,t}^{(3)} 在全量任务上汇总即为主表指标 VHDR
\todo{Clarify .}

\paragraph{Failure-Aware Refinement Agent.}
\label{sec:failure_aware_refinement}

A quality-approved question may still be too weak to expose the target VLM,
and independent regeneration does not exploit information revealed by the
previous response. The \emph{Failure-Aware Refinement Agent} therefore
diagnoses why a valid candidate failed to elicit hallucination and converts
the observed response into targeted revision instructions.

When $Q_{i,t}=1$ and $H_{i,t}^{(3)}=0$, the agent analyzes the fixed
configuration $z_i$, candidate question $q_{i,t}$, elicitation content
$\rho_{i,t}$, target-model response $\hat{y}_{i,t}$, and judge score
$j_{i,t}$:
\begin{equation}
F_{i,t}^{\mathrm{tar}}
=
\operatorname{FAR}
\left(
z_i,
q_{i,t},
\rho_{i,t},
\hat{y}_{i,t},
j_{i,t}
\right),
\end{equation}
where $F_{i,t}^{\mathrm{tar}}$ contains target-oriented revision instructions
for the Composer. The revision may adjust the visual focus, manipulated
premise, wording, answer options, elicitation strength, or realization of the
prescribed format, while keeping $s_i$, $w_i$, and $f_i$ fixed.

SEAM performs one initial attempt and, when necessary, one
feedback-guided retry. Quality-invalid candidates use feedback from the
Hierarchical Question Verifier, whereas quality-approved candidates that fail
to elicit hallucination use $F_{i,1}^{\mathrm{tar}}$. After at most two
attempts, the validity-first rule selects the final candidate, which is added
to the corresponding target-specific question bank if quality-approved.



\subsection{Evidence-Guided Skill Evolution}
\label{sec:skill_evolution}
As shown in Figure~1, the Skill Updater proposes local edits from
inner-loop training trajectories stored in the Training Trajectory
Memory. Edits passing static checks and validation update the Shared
Skill Library. Updated skills guide content selection (e.g., objects,
attributes, and relations), question construction, and reference-answer
verification, aiming to increase VHDR while maintaining question quality
and evaluation reliability. The library is frozen before testing.

\paragraph{Training Trajectory Memory.}
We partition the image pool into training, validation, and test splits
for proposing edits, selecting updates, and final evaluation, respectively.
All model weights remain frozen. The memory stores historical training
trajectories generated using $\mathcal{S}^{0}$, including questions,
reference answers, quality feedback, revision histories, and target
responses and hallucination judgments when available.
We preserve each task's complete attempt history and organize usable
feedback into three evidence streams: quality failures, quality-approved
attempts without hallucinations, and quality-approved attempts with
hallucinations. Different attempts from the same task may contribute
to different streams. Records involving disputed judgments, review
flags, or execution errors are retained for traceability but excluded
from definitive editing evidence.

\paragraph{Local Skill Editing.}
Given a skill $s$ and its textual training trajectories $\mathcal{T}_s$,
the Skill Updater $\mathcal{U}$ performs batch reflection to propose
local edits, within-stream consolidation to merge recurring suggestions,
and cross-stream consolidation to resolve conflicts, prioritizing
quality corrections. Each stage uses the original skill and complete
configuration definitions. Each candidate contains at most two edits,
each supported by at least three distinct tasks.
Only probing rules are editable; type definitions, wrapper definitions
and bindings, and format specifications remain fixed.
Configuration-specific recommendations retain their scope, while general
verification edits require quality-failure evidence and type-definition
support. Static checks verify evidence references and edit constraints.

\paragraph{Validation and Acceptance.}
Candidates are compared with the original skills using the same
validation tasks, attempt budget, and frozen evaluation criteria.
The quality pass rate $Q_{\mathrm{val}}$ and VHDR $V_{\mathrm{val}}$
both use all assigned tasks as the denominator.
A candidate $s'$ is accepted only if evaluation completes without
evaluation errors, review and execution-error rates do not increase,
and
\begin{equation}
\begin{aligned}
Q_{\mathrm{val}}(s') &\geq Q_{\mathrm{val}}(s), \\
V_{\mathrm{val}}(s') &\geq V_{\mathrm{val}}(s) + \delta,
\end{aligned}
\label{eq:skill_acceptance}
\end{equation}
where both rates lie in $[0,1]$ and $\delta=0.01$.
Each skill is accepted independently or retains its original version.
The resulting library $\mathcal{S}^{*}$ is frozen before testing,
with test feedback restricted to within-task refinement.
All edits, supporting evidence, and validation decisions are recorded.
